Pushdown Normal-Form Bisimulation: A Nominal Context-Free Approach to Program Equivalence

We propose Pushdown Normal Form (PDNF) Bisimulation to verify contextual equivalence in higher-order functional programming languages with local state. Similar to previous work on Normal Form (NF) bisimulation, PDNF Bisimulation is sound and complete with respect to contextual equivalence. However, unlike traditional NF Bisimulation, PDNF Bisimulation is also decidable for a class of program terms that reach bounded configurations but can potentially have unbounded call stacks and input an unbounded number of unknown functions from their context. Our approach relies on the principle that, in model-checking for reachability, pushdown systems can be simulated by finite-state automata designed to accept their initial/final stack content. We embody this in a stackless Labelled Transition System (LTS), together with an on-the-fly saturation procedure for call stacks, upon which bisimulation is defined. To enhance the effectiveness of our bisimulation, we develop up-to techniques and confirm their soundness for PDNF Bisimulation. We develop a prototype implementation of our technique which is able to verify equivalence in examples from practice and the literature that were out of reach for previous work.

==> soundness.tex <==


\subsection{Up to Fold}

\begin{definition}[Concretisation]
  A \emph{concretisation} $\concr{\alpha}{v}$
  is defined when $\alpha\not\in\an{v}$, and we
  write $e\concr{\alpha}{v}$ for the expression obtained after substituting $\alpha$ for $v$ in $e$.
  We let $\dom{\concr{\alpha}{v}}=\{\alpha\}$ and $\rng{\concr{\alpha}{v}}=\{v\}$,
  and let $\kappa$ range over concretisations.
  We lift concretisation to contexts, environments and stores point-wise; we also lift it to configurations, writing
  $C\kappa$
  to mean $\conf{A\sdif\dom{\kappa}}{\Gamma\kappa}{K\kappa}{s\kappa}{e\kappa}$, when $C=\conf{A}{\Gamma}{K}{s}{e}$.
  \defqed
\end{definition}

\begin{figure*}[t] %{{{
  \[\begin{array}{@{}c@{}}
    \irule[UTFe1][utfe1]{
      \conf{A_1}{\Gamma_1}{E_1,K_1}{s_1}{e_1}
      \bisim*{R}
      \conf{A_2}{\Gamma_2}{E_2,K_2}{s_2}{e_2}
    }{
      \conf{A_1}{\Gamma_1}{K_1}{s_1}{E_1\hole[e_1]}
      \utfolde*{\bisim{R}}
      \conf{A_2}{\Gamma_2}{K_2}{s_2}{E_2\hole[e_2]}
    }
    \\\\
    \irule[UTFe2][utfe2]{
      \conf{A_1}{\Gamma_1}{K_{11},E_1,E'_1,K_{12}}{s_1}{\hat e_1}
      \bisim*{R}
      \conf{A_2}{\Gamma_2}{K_{21},E_2,E'_2,K_{22}}{s_2}{\hat e_2}
      \\
      \sizeof{K_{11}}=\sizeof{K_{21}}
    }{
      \conf{A_1}{\Gamma_1}{K_{11},E'_1\hole[E_1],K_{12}}{s_1}{\hat e_1}
      \utfolde*{\bisim{R}}
      \conf{A_2}{\Gamma_2}{K_{21},E'_2\hole[E_2],K_{22}}{s_2}{\hat e_2}
    }
    \\\\
    \irule[UTFd1][utfd1]{
      \conf{A_1}{\Gamma_1}{E_1,K_1}{s_1}{e_1}
      \bisim*{R}
      \botconf
    }{
      \conf{A_1}{\Gamma_1}{K_1}{s_1}{E_1\hole[e_1]}
      \utfolde*{\bisim{R}}
      \botconf
    }
    \quad
    \irule[UTFd2][utfd2]{
      \conf{A_1}{\Gamma_1}{K_{11},E_1,E'_1,K_{12}}{s_1}{\hat e_1}
      \bisim*{R}
      \botconf
    }{
      \conf{A_1}{\Gamma_1}{K_{11},E'_1\hole[E_1],K_{12}}{s_1}{\hat e_1}
      \utfolde*{\bisim{R}}
      \botconf
    }
  \end{array}\]
    \Hline
  \[\begin{array}{@{}c@{}}
     \irule[UTFv][utfv]{
       \conf{A_1\uplus\alpha}{\Gamma_1,\maps{i}{v_1}}{K_1}{s_1}{\hat e_1}
      \bisim*{R}
      \conf{A_2\uplus\alpha}{\Gamma_2,\maps{i}{v_2}}{K_2}{s_2}{\hat e_2}
      \\\\
      \kappa_1=\concr{\alpha}{v_1}
      \\
      \kappa_2=\concr{\alpha}{v_2}
      \\
      \alpha\not\in\an{v_1,v_2}
    }{
      \conf{A_1}{\Gamma_1\kappa_1}{K_1\kappa_1}{s_1\kappa_1}{\hat e_1\kappa_1}
      \utfoldv*{\bisim{R}}
      \conf{A_2}{\Gamma_2\kappa_2}{K_2\kappa_2}{s_2\kappa_2}{\hat e_2\kappa_2}
    }
   \\\\
    \irule[UTFd3][utfd3]{
      \conf{A_1\uplus\alpha}{\Gamma_1,\maps{i}{v_1}}{K_1}{s_1}{\hat e_1}
      \bisim*{R}
      \botconf
      \\
      \kappa_1=\concr{\alpha}{v_1}
      \\
      \alpha\not\in\an{v_1}
    }{
      \conf{A_1}{\Gamma_1\kappa_1}{K_1\kappa_1}{s_1\kappa_1}{\hat e_1\kappa_1}
      \utfoldv*{\bisim{R}}
      \botconf
    }
  \end{array}\]
  \hrule
  \caption{Up-to fold.}\label{fig:utfold}
\end{figure*}
%}}}

\begin{lemma}\label{lem:utfolde-sound} %{{{
  Let $f= \utfolde{}\sqcup\utfoldv{}$; then
  %and $g=\utId{}$; then
  $\utfolde{}\comp{\constf{\gfp\WP}}\progress f^\omega\comp{\constf{\gfp\WP}}$.
\end{lemma}
\begin{proof}
  We need to show
  $\utfolde{}\comp{\constf{\gfp\WP}}\comp\WP(\bisim{R}) \sqsubseteq 
  {\WP}\comp f^\omega\comp{\constf{\gfp\WP}}(\bisim{R})$.
  Because $\constf{\gfp\WP}$ is the constant function mapping its argument to $(\simil)$, we need to show
  $\utfolde{}(\simil) \sqsubseteq 
  {\WP}\comp f^\omega(\simil)$.

  Let $C_1\utfolde*{\simil}C_2$, 
  and $C_1\trans{\eta}C_1'$.
  If $C_1\trans{\eta}C_1'$ is produced by rule \iref{dummy} then the proof is trivial as $C_2$ can perform the same transition and $C_1'=\botconf \mathrel{f^0(\simil)} \botconf=C_2'$. We thus consider only non-\iref{dummy} transitions from $C_1$.
  We proceed by case analysis on the derivation
  $C_1\utfolde*{\simil}C_2$.


  {\flushleft
  \iref{utfe1}:}
  $C_1=\conf{A_1}{\Gamma_1}{K_1}{s_1}{E_1\hole[e_1]}$ and
  $C_2=\conf{A_2}{\Gamma_2}{K_2}{s_2}{E_2\hole[e_2]}$ and
  $C_3=\conf{A_1}{\Gamma_1}{E_1,K_1}{s_1}{e_1}$ and
  $C_4=\conf{A_2}{\Gamma_2}{E_2,K_2}{s_2}{e_2}$ and
  $C_3 \mathrel{\simil} C_4$.
  In this case $C_1$ is a proponent configuration thus the transition can only be produced by rules
  \iref{propappf}, \iref{propretf}, and \iref{tau}.

  \begin{itemize}
    \item
      \iref{propappf}: Here we show only the case for the latter rule.
      We have $\eta=\lpropapp{\alpha}{i}$ and
      $E_1\hole[e_1] = E\hole[\app \alpha v]$
      and
      $C'_1=\conf{A_1}{\Gamma_1,\maps{i}{v_1}}{E_1';K_1}{s_1}{\noe}$.
      We have the following three cases:
      \begin{itemize}
        \item $e_1=E_1'\hole[\app\alpha v_1]$, $E=E_1\hole[E_1'\hole]]$:
          In this case configuration $C_3$ can perform the same transition:
          $C_3\trans{\eta}C_3'=\conf{A_1}{\Gamma_1,\maps{i}{v_1}}{E_1',E_1,K}{s_1}{\noe}$.
          Because $C_3\simil C_4$,
          $C_4\wtrans{\eta}C_4'=\conf{A_2}{\Gamma_2'}{E_2',E_2,K}{s_2'}{\noe}$ or
          $C_4\wtrans{\eta}C_4'=\botconf$, and $C_3'\simil C_4'$.
          In the case where $C_4$ goes to \botconf, $C_2\trans{\eta}\botconf$ and
          $C_1' \utfolde*{\simil} \botconf$ by rule \iref{utfd2}.
          In the other case we derive $C_2\wtrans{\eta}C_2'=\conf{A_2}{\Gamma_2'}{E_2\hole[E_2']}{s_2'}{\noe}$
          and $C_1' \utfolde*{\bisim{S}} C_2'$ by rule \iref{utfe2}.

        \item $e_1=\alpha$, $E_1=E_1'\hole[\app\hole v_1]$
      and $C'_1=\conf{A_1}{\Gamma_1,\maps{i}{v_1}}{E_1';K_1}{s_1}{\noe}$:

          In this case configuration $C_3$ can perform the transitions:
          \begin{align*}
            C_3
            &\trans{\lpropret{j}}
            \conf{A_1}{\Gamma_1,\maps{j}{\alpha}}{E_1'\hole[\app\hole v_1],K_1}{s_1}{\noe}
            \\&\trans{\lopret{\alpha'}}
            \conf{A_1\uplus\alpha'}{\Gamma_1,\maps{j}{\alpha}}{K_1}{s_1}{E_1'\hole[\app\alpha' v_1]}
            \\&\trans{\lpropapp{\alpha'}{j'}}
            \conf{A_1\uplus\alpha'}{\Gamma_1,\maps{j}{\alpha},\maps{j'}{v_1}}{E_1',K_1}{s_1}{\noe}
            &(\alpha'\not\in\an{\Gamma_1,K_1,s_1,E_1',v_1})
            \\&\trans{\lopapp{j}{\alpha''}}
            \conf{A_1\uplus\alpha',\alpha''}{\Gamma_1,\maps{j}{\alpha},\maps{j'}{v_1}}{E_1',K_1}{s_1}{\app\alpha{\alpha''}}
            &(\alpha''\not\in\an{\Gamma_1,K_1,s_1,E_1',v_1})
            \\&\trans{\lpropapp{\alpha}{i}}
            \conf{A_1\uplus\alpha',\alpha''}{\Gamma_1,\maps{j}{\alpha},\maps{j'}{v_1},\maps{i}{\alpha''}}{
              \hole,E_1',K_1}{s_1}{\noe}
            =C_3'
          \end{align*}
          Because $C_3\simil C_4$, there exists $C_4'$ such that
          \[
            C_4
            \wtrans{\lpropret{j}}
            \wtrans{\lopret{\alpha'}}
            \wtrans{\lpropapp{\alpha'}{j'}}
            \wtrans{\lopapp{j}{\alpha''}}
            \wtrans{\lpropapp{\alpha}{i}}
            C_4'
          \]
          and $C_3' \simil C_4'$. By analysis of the transitions we have two possibilities:
          \begin{itemize}
            \item $C_4'=\botconf$ and in this case we have
              $C_2 \trans{\eta}\botconf$.
             Moreover:
             \begin{align*}
               C_3'&=
               \conf{A_1\uplus\alpha',\alpha''}{\Gamma_1,\maps{j}{\alpha},\maps{j'}{v_1},\maps{i}{\alpha''}}{
               \hole,E_1',K_1}{s_1}{\noe}
               \simil \botconf
              \\
               &\mathrel{\phantom{=}}
               \conf{A_1\uplus\alpha',\alpha''}{\Gamma_1,\maps{i}{\alpha''}}{
               \hole,E_1',K_1}{s_1}{\noe}
               \concr{\alpha''}{v_1}
               \concr{\alpha'}{\alpha}
               \utfoldv*{\utfoldv{\simil}}
               \botconf
              &\text{(\iref{utfd3})}
              \\
               &\mathrel{\phantom{=}}
               \conf{A_1}{\Gamma_1,\maps{i}{v_1}}{
               \hole,E_1',K_1}{s_1}{\noe}
               \utfoldv*{\utfoldv{\simil}}
               \botconf
               &\hspace{18ex}
               \llap{$(\alpha',\alpha''\not\in\an{\Gamma_1,K_1,s_1,E_1',v_1})$}
              \\
               C_1'&=\conf{A_1}{\Gamma_1,\maps{i}{v_1}}{
               E_1'\hole,K_1}{s_1}{\noe}
              \utfolde*{\utfoldv{\utfoldv{\simil}}}
               \botconf
              &\text{(\iref{utfe2})}
              \end{align*}

            \item
              Otherwise we have:
             \begin{align*}
               C_4 & =\conf{A_2}{\Gamma_2}{E_2,K_2}{s_2}{e_2}
               \wtrans{\tau}
              \conf{A_2}{\Gamma_2}{E_2,K_2}{s_2'}{w_2}
              \\& \trans{\lpropret{j}}
               \conf{A_2}{\Gamma_2,\maps{j}{w_2}}{E_2,K_2}{s_2'}{\noe}
               \\&\trans{\lopret{\alpha'}}
              \conf{A_2\uplus\alpha'}{\Gamma_2,\maps{j}{w_2}}{K_2}{s_2'}{E_2\hole[\alpha']}
               &(\alpha'\not\in\an{\Gamma_2,K_2,w_2})
              \\& \wtrans{\tau}
              \conf{A_2\uplus\alpha'}{\Gamma_2,\maps{j}{w_2}}{K_2}{s_2''}{E_2'\hole[\app\alpha' w_2']}
              \\&\trans{\lpropapp{\alpha'}{j'}}
              \conf{A_1\uplus\alpha'}{\Gamma_2,\maps{j}{w_2},\maps{j'}{w_2'}}{E'_2,K_2}{s_2''}{\noe}
              \\&\trans{\lopapp{j}{\alpha''}}
               \conf{A_1\uplus\alpha',\alpha''}{\Gamma_2,\maps{j}{w_2},\maps{j'}{w_2'}}{E'_2,K_2}{s_2''}{\app{w_2}{\alpha''}}
               &(\alpha''\not\in\an{w_2'})
              \\& \wtrans{\tau}
               \conf{A_1\uplus\alpha',\alpha''}{\Gamma_2,\maps{j}{w_2},\maps{j'}{w_2'}}{E'_2,K_2}{s_2''}{E''_2\hole[\app{\alpha}{v_2}]}
              \\&\trans{\lpropapp{\alpha}{i}}
               \conf{A_1\uplus\alpha',\alpha''}{\Gamma_2,\maps{j}{w_2},\maps{j'}{w_2'},\maps{i}{v_2'}}{
                 E''_2,E'_2,K_2}{s_2''}{\noe}
               =C_4'
             \end{align*}
              Using \cref{lem:lts-concr} and LTS rule $\iref{tau}$, we can derive the following transitions from $C_2$:
             \begin{align*}
               C_2 & =\conf{A_2}{\Gamma_2}{K_2}{s_2}{E_2\hole[e_2]}
               \wtrans{\tau}
               \conf{A_2}{\Gamma_2}{K_2}{s_2'}{E_2\hole[w_2]}
              \\& =
               \conf{A_2\uplus\alpha'}{\Gamma_2}{K_2}{s_2'}{E_2\hole[\alpha']}\concr{\alpha'}{w_2}
               &(\alpha'\not\in\an{w_2})
              \\& \wtrans{\tau}
               \conf{A_2\uplus\alpha'}{\Gamma_2}{K_2}{s_2''}{E_2'\hole[\app\alpha' w_2']}\concr{\alpha'}{w_2}
              \\&=
               \conf{A_1\uplus\alpha',\alpha''}{\Gamma_2}{K_2}{s_2''}{E'_2\hole[\app{w_2}{\alpha''}]}
               \concr{\alpha''}{w_2'}
               \concr{\alpha'}{w_2}
               &(\alpha''\not\in\an{w_2'})
              \\& \wtrans{\tau}
               \conf{A_1\uplus\alpha',\alpha''}{\Gamma_2}{,K_2}{s_2''}{
                 E'_2\hole[E''_2\hole[\app{\alpha}{v_2}]]}
               \concr{\alpha''}{w_2'}
               \concr{\alpha'}{w_2}
              \\&\trans{\lpropapp{\alpha}{i}}
               \conf{A_1\uplus\alpha',\alpha''}{\Gamma_2,\maps{i}{v_2}}{
                 E'_2\hole[E''_2],K_2}{s_2''}{\noe}
               \concr{\alpha''}{w_2'}
               \concr{\alpha'}{w_2}
               =C_2'
             \end{align*}
             We also have
             \[\abox{
               C_3'&=
               \conf{A_1\uplus\alpha',\alpha''}{\Gamma_1,\maps{j}{\alpha},\maps{j'}{v_1},\maps{i}{\alpha''}}{
               \hole,E_1',K_1}{s_1}{\noe}
             \\&\simil
               \conf{A_1\uplus\alpha',\alpha''}{\Gamma_2,\maps{j}{w_2},\maps{j'}{w_2'},\maps{i}{v_2'}}{
               E''_2,E'_2,K_2}{s_2''}{\noe}
               =C_4'
             }\]
             By rule \iref{utfv}
             \[\nbox{
               \conf{A_1\uplus\alpha',\alpha''}{\Gamma_1,\maps{i}{\alpha''}}{
               \hole,E_1',K_1}{s_1}{\noe}
               \concr{\alpha''}{v_1}
               \concr{\alpha'}{\alpha}
               \\\quad\utfoldv*{\utfoldv{\simil}}
               \conf{A_1\uplus\alpha',\alpha''}{\Gamma_2,\maps{i}{v_2'}}{
               E''_2,E'_2,K_2}{s_2''}{\noe}
               \concr{\alpha''}{w_2'}
               \concr{\alpha'}{w_2}
             }\]
            Because $\alpha',\alpha''\not\in\an{\Gamma_1,K_1,s_1,E_1',v_1}$
             \[\nbox{
               \conf{A_1}{\Gamma_1,\maps{i}{v_1}}{
               \hole,E_1',K_1}{s_1}{\noe}
               \\\quad\utfoldv*{\utfoldv{\simil}}
               \conf{A_1\uplus\alpha',\alpha''}{\Gamma_2,\maps{i}{v_2'}}{
               E''_2,E'_2,K_2}{s_2''}{\noe}
               \concr{\alpha''}{w_2'}
               \concr{\alpha'}{w_2}
             }\]
             By rule \iref{utfe2}
             \[\nbox{
               \conf{A_1}{\Gamma_1,\maps{i}{v_1}}{
               E_1'\hole,K_1}{s_1}{\noe}
             \\\quad\utfolde*{\utfoldv{\utfoldv{\simil}}}
               \conf{A_1\uplus\alpha',\alpha''}{\Gamma_2,\maps{i}{v_2'}}{
                 E'_2\hole[E''_2],K_2}{s_2''}{\noe}
               \concr{\alpha''}{w_2'}
               \concr{\alpha'}{w_2}
             }\]
             Therefore $C_1' \utfolde*{\utfoldv{\utfoldv{\simil}}} C_2'$ as required.
           \end{itemize}

        \item $e_1=v_1$, $E_1=E_1'\hole[\app\alpha\hole]$
            and $C'_1=\conf{A_1}{\Gamma_1,\maps{i}{v_1}}{E_1';K_1}{s_1}{\noe}$:
          In this case configuration $C_3$ can perform the transitions:
          \begin{align*}
            C_3
            &\trans{\lpropret{j}}
            \conf{A_1}{\Gamma_1,\maps{j}{v}}{E_1'\hole[\app\alpha\hole],K_1}{s_1}{\noe}
            \\&\trans{\lopret{\alpha'}}
            \conf{A_1\uplus\alpha'}{\Gamma_1,\maps{j}{v}}{K_1}{s_1}{E_1'\hole[\app\alpha\alpha']}
            &(\alpha'\not\in\an{\Gamma_1,v_1,K_1,s_1,E_1'})
            \\&\trans{\lpropapp{\alpha}{i}}
            \conf{A_1\uplus\alpha'}{\Gamma_1,\maps{j}{v},\maps{i}{\alpha'}}{E_1',K_1}{s_1}{\noe}
            =C_3'
          \end{align*}
          Because $C_3\simil C_4$, there exists $C_4'$ such that
          $C_4
            \wtrans{\lpropret{j}}
            \wtrans{\lopret{\alpha'}}
            \wtrans{\lpropapp{\alpha}{i}}
          C_4'$
          and $C_3' \simil C_4'$. By analysis of the transitions we have
          \begin{align*}
            C_4 & =\conf{A_2}{\Gamma_2}{E_2,K_2}{s_2}{e_2}
            \wtrans{\tau}
            \conf{A_2}{\Gamma_2}{E_2,K_2}{s_2'}{v_2}
            \\& \trans{\lpropret{j}}
            \conf{A_2}{\Gamma_2,\maps{j}{v_2}}{E_2,K_2}{s_2'}{\noe}
            \\& \trans{\lopret{ \alpha'}}
            \conf{A_2\uplus\alpha'}{\Gamma_2,\maps{j}{v_2}}{K_2}{s_2'}{E_2\hole[\alpha']}
            &(\alpha'\not\in\an{\Gamma_2,v_2,K_2,s_2',E_2'})
            \\& \wtrans{\tau}
            \conf{A_2\uplus\alpha'}{\Gamma_2,\maps{j}{v_2}}{K_2}{s_2''}{E_2'\hole[\app \alpha w_2]}
            &
            \\& \trans{\lpropapp{\alpha}{i}}
            \conf{A_2\uplus\alpha'}{\Gamma_2,\maps{j}{v_2},\maps{i}{w_2}}{E_2',K_2}{s_2''}{\noe}
            = C_4'
          \end{align*}
          Using \cref{lem:lts-concr} and LTS rule $\iref{tau}$, we can derive the following transitions from $C_2$:
          \begin{align*}
            C_2 & =\conf{A_2}{\Gamma_2}{K_2}{s_2}{E_2\hole[e_2]}
            \wtrans{\tau}
            \conf{A_2}{\Gamma_2}{K_2}{s_2'}{E_2[v_2]}
            \\&=
            \conf{A_2\uplus\alpha'}{\Gamma_2}{K_2}{s_2'}{E_2\hole[\alpha']}
            \concr{\alpha'}{v_2}
            \wtrans{\tau}
            \conf{A_2\uplus\alpha'}{\Gamma_2}{K_2}{s_2''}{E_2'\hole[\app \alpha w_2]}
            \concr{\alpha'}{v_2}
            &
            \\& \trans{\lpropapp{\alpha}{i}}
            \conf{A_2\uplus\alpha'}{\Gamma_2,\maps{i}{w_2}}{E_2',K_2}{s_2''}{\noe}
            \concr{\alpha'}{v_2}
            = C_2'
          \end{align*}
          We also have
          \[
            C_3' =
            \conf{A_1\uplus\alpha'}{\Gamma_1,\maps{j}{v},\maps{i}{\alpha'}}{E_1',K_1}{s_1}{\noe}
            \simil
            \conf{A_2\uplus\alpha'}{\Gamma_2,\maps{j}{v_2},\maps{i}{w_2}}{E_2',K_2}{s_2''}{\noe}
            = C_4'
          \]
          And by rule \iref{utfv}:
          \[\abox{
            C_1' &=
            \conf{A_1}{\Gamma_1,\maps{i}{v_1}}{E_1',K_1}{s_1}{\noe}
            \\&=
            \conf{A_1\uplus\alpha'}{\Gamma_1,\maps{i}{\alpha'}}{E_1',K_1}{s_1}{\noe}
            \concr{\alpha'}{v_1}
            \utfoldv*{\simil}
            \conf{A_2\uplus\alpha'}{\Gamma_2,\maps{i}{w_2}}{E_2',K_2}{s_2''}{\noe}
            \concr{\alpha'}{v_2}
            = C_2'
          }\]
 
      \end{itemize}
    \item
      \iref{propretf}: here we show only the case for the latter rule.
      We have $\eta=\lpropret{i}$ and $E_1=\hole$
      and $C'_1=\conf{A_1}{\Gamma_1,\maps{i}{v_1}}{K_1}{s_1}{\noe}$.
      Configuration $C_3$ can perform the transitions:
      \begin{align*}
        C_3
        &\trans{\lpropret{j}}
        \conf{A_1}{\Gamma_1,\maps{j}{v_1}}{\hole,K_1}{s_1}{\noe}
        \\&\trans{\lopret{\alpha'}}
        \conf{A_1\uplus\alpha'}{\Gamma_1,\maps{j}{v_1}}{K_1}{s_1}{\hole[\alpha']}
        &(\alpha'\not\in\an{\Gamma_1,v_1,K_1,s_1})
        \\&\trans{\lpropret{i}}
        \conf{A_1\uplus\alpha'}{\Gamma_1,\maps{j}{v_1},\maps{i}{\alpha'}}{K_1}{s_1}{\noe}
        =C_3'
      \end{align*}
      Because $C_3\simil C_4$, there exists $C_4'$ such that
      $C_4
        \wtrans{\lpropret{j}}
        \wtrans{\lopret{\alpha'}}
        \wtrans{\lpropret{i}}
      C_4'$
      and $C_3' \simil C_4'$. By analysis of the transitions we have
      \begin{align*}
        C_4 &=
        \conf{A_2}{\Gamma_2}{E_2,K_1}{s_1}{e_2}
        \wtrans{\tau}
        \conf{A_2}{\Gamma_2}{E_2,K_1}{s_1'}{v_2}
        \\&\trans{\lpropret{j}}
        \conf{A_2}{\Gamma_2,\maps{j}{v_2}}{E_2,K_2}{s_2'}{\noe}
        \\&\trans{\lopret{\alpha'}}
        \conf{A_2\uplus\alpha'}{\Gamma_2,\maps{j}{v_2}}{K_2}{s_2'}{E_2\hole[\alpha']}
        &(\alpha'\not\in\an{\Gamma_2,v_2,K_2,s_2',E_2})
        \\&\wtrans{\tau}
        \conf{A_2\uplus\alpha'}{\Gamma_2,\maps{j}{v_2}}{K_2}{s_2''}{w_2}
        \\&\trans{\lpropret{i}}
        \conf{A_2\uplus\alpha'}{\Gamma_2,\maps{j}{v_2},\maps{i}{w_2}}{K_2}{s_2''}{\noe}
        =C_4'
      \end{align*}
      Using \cref{lem:lts-concr} and LTS rule $\iref{tau}$, we can derive the following transitions from $C_2$:
      \begin{align*}
        C_2 &=
        \conf{A_2}{\Gamma_2}{K_1}{s_1}{E_2\hole[e_2]}
        \wtrans{\tau}
        \conf{A_2}{\Gamma_2}{K_1}{s_1'}{E_2\hole[v_2]}
        \\&=
        \conf{A_2\uplus\alpha'}{\Gamma_2}{K_2}{s_2'}{E_2\hole[\alpha']}
        \concr{\alpha'}{v_2}
        \wtrans{\tau}
        \conf{A_2\uplus\alpha'}{\Gamma_2}{K_2}{s_2''}{w_2}
        \concr{\alpha'}{v_2}
        \\&\trans{\lpropret{i}}
        \conf{A_2\uplus\alpha'}{\Gamma_2,\maps{i}{w_2}}{K_2}{s_2''}{\noe}
        \concr{\alpha'}{v_2}
        =C_2'
      \end{align*}
      Moreover,
      \[\abox{
        C_1' &= \conf{A_1}{\Gamma_1,\maps{i}{v_1}}{K_1}{s_1}{\noe}
        \\ &= \conf{A_1\uplus\alpha'}{\Gamma_1,\maps{i}{\alpha'}}{K_1}{s_1}{\noe} \concr{\alpha'}{v_1}
        \utfoldv*{\simil}
        \conf{A_2\uplus\alpha'}{\Gamma_2,\maps{i}{w_2}}{K_2}{s_2''}{\noe}\concr{\alpha'}{v_2}
        =C_2'
      }\]
 

    \item
      \iref{tau}:
      We have $\eta=\tau$ and 
      and $C'_1=\conf{A_1}{\Gamma_1}{K_1}{s_1'}{e_1'}$
      and $\redconf{s_1}{E_1\hole[e_1]} \red \redconf{s_1'}{e_1'}$.
      By the reduction rule we get $E_1\hole[e_1]=E\hole[e]$ and 
      $\redconf{s_1}{e} \redbase \redconf{s_1'}{e'}$ and $e_1'=E\hole[e']$, for some $E,e,e'$.

      We proceed by cases on $E_1\hole[e_1]=E\hole[e]$:
      \begin{itemize}
        \item $e_1=E_{e_1}\hole[e]$ and $E=E_1\hole[E_{e_1}\hole]$ and $e_1'=E_1\hole[{E_{e_1}\hole[e']}]$.
          In this case $C_3$ can perform the same transition:
          \[
            C_3 = \conf{A_1}{\Gamma_1}{E_1,K_1}{s_1}{E_{e_1}\hole[e]}
            \trans{\tau} \conf{A_1}{\Gamma_1}{E_1,K_1}{s_1'}{E_{e_1}\hole[e']} = C_3'
          \]
          Because $C_3 \simil C_4$,
          \[
            C_4 = \conf{A_2}{\Gamma_2}{E_2,K_2}{s_2}{e_2}
            \wtrans{\tau} \conf{A_2}{\Gamma_2}{E_2,K_2}{s_2'}{e_2'} = C_4'
          \]
          and $C_3' \simil C_4'$. Therefore
          \[
            C_2 = \conf{A_2}{\Gamma_2}{K_2}{s_2}{E_2\hole[e_2]}
            \wtrans{\tau} \conf{A_2}{\Gamma_2}{K_2}{s_2'}{E_2\hole[e_2']} = C_2'
          \]
          and from rule \iref{utfe1}, $C_1' \utfolde*{\simil} C_2'$.

        \item $e_1=v_1$ and $E_1=E\hole[F]$
          and
          $\redconf{s_1}{F\hole[v_1]} \redbase \redconf{s_1'}{e'}$,
          where $F$ is one of the following contexts:
          $(\arithop{\vec c_{11},\hole,\vec c_{12}})$ or
          $(\app \hole v)$ or
          $(\app v \hole)$ or
          $(l \asgn \hole)$ or
          $(\cond \hole{e_{11}}{e_{12}})$.
          We proceed by cases on $F$:
          \begin{itemize}
            \item $F=\arithop{\vec c_{11},\hole,\vec c_{12}}$:
              Here it must be $v_1=c$ and $e'=c'=\arithop{\vec c_{11},c,\vec c_{12}}$. Thus $C_3$ can perform the transitions
              \begin{align*}
                C_3 &= \conf{A_1}{\Gamma_1}{E\hole[F],K_1}{s_1}{c}
                \trans{\lpropret{c}}
                \conf{A_2}{\Gamma_1}{E\hole[F],K_1}{s_1}{\noe}
                \\&\trans{\lopret{c}}
                \conf{A_2}{\Gamma_1}{K_1}{s_1}{E\hole[F{\hole[c]}]}
                \trans{\tau}
                \conf{A_2}{\Gamma_1}{K_1}{s_1}{E\hole[c']}
                =C_3' = C_1'
              \end{align*}
              Because $C_3 \simil C_4$,
              \begin{align*}
                C_4 &= \conf{A_2}{\Gamma_2}{E_2,K_2}{s_2}{e_2}
                \wtrans{\tau}
                \conf{A_2}{\Gamma_2}{E_2,K_2}{s_2'}{c}
                \trans{\lpropret{c}}
                \conf{A_2}{\Gamma_2}{E_2,K_2}{s_2'}{\noe}
                \\&\trans{\lopret{c}}
                \conf{A_2}{\Gamma_2}{K_2}{s_2'}{E_2\hole[c]}
                \wtrans{\tau}
                C_4'
              \end{align*}
              and $C_3'\simil C_4'$. Moreover we derive the transitions:
              \begin{align*}
                C_2 &= \conf{A_2}{\Gamma_2}{K_2}{s_2}{E_2\hole[e_2]}
                \wtrans{\tau}
                \conf{A_2}{\Gamma_2}{K_2}{s_2'}{E_2\hole[c]}
                \wtrans{\tau}
                C_4' = C_2'
              \end{align*}
              We also derive $C_1' \mathrel{f^0(\simil)} C_2'$ as needed.
             
            \item $F=\app \hole v$: Here it must be $v_1 = \lam{x} e_{11}$ and $e'=e_{11}\sub{x}{v}$.
              By the LTS and $C_3\simil C_3'$ we have:
             \begin{align*}
               C_3 &= \conf{A_1}{\Gamma_1}{E\hole[F],K_1}{s_1}{\lam{x} e_{11}}
                \\&\trans{\lpropret{i}}
                \conf{A_2}{\Gamma_1,\maps{i}{\lam{x} e_{11}}}{E\hole[F],K_1}{s_1}{\noe}
                \\&\trans{\lopret{\alpha}}
                \conf{A_1\uplus\alpha}{\Gamma_1,\maps{i}{\lam{x} e_{11}}}{K_1}{s_1}{E\hole[\app\alpha v]}
                &(\alpha\not\in\an{A_1,\Gamma_1,e_{11},K_1,s_1,E,v})
                \\&\trans{\lpropapp{\alpha}{j}}
                \conf{A_1\uplus\alpha}{\Gamma_1,\maps{i}{\lam{x} e_{11},\maps{j}{v}}}{E,K_1}{s_1}{\noe}
                \\&\trans{\lopapp{i}{\alpha'}}
                \conf{A_1\uplus\alpha}{\Gamma_1,\maps{i}{\lam{x} e_{11},\maps{j}{v}}}{E,K_1}{s_1}{e_{11}\sub{x}{\alpha'}}
                =C_3'
                &(\alpha'\not\in\an{A_1,\Gamma_1,e_{11},K_1,s_1,E,v})
             \end{align*}
             %\begin{align*}
             %  C_3 &= \conf{A_1}{\Gamma_1}{E\hole[F],K_1}{s_1}{\lam{x} e_{11}}
             %   \\&\trans{\lpropret{i}}
             %   \conf{A_2}{\Gamma_1,\maps{i}{\lam{x} e_{11}}}{E\hole[F],K_1}{s_1}{\noe}
             %   \\&\trans{\lopret{\alpha}}
             %   \conf{A_1\uplus\alpha}{\Gamma_1,\maps{i}{\lam{x} e_{11}}}{K_1}{s_1}{E\hole[\app\alpha v]}
             %   =C_3'
             %   &(\alpha\not\in\an{A_1,\Gamma_1,e_{11},K_1,s_1,E,v})
             %\end{align*}
             \begin{align*}
               C_4 &= \conf{A_2}{\Gamma_2}{E_2,K_2}{s_2}{e_2}
                \wtrans{\tau}
                \conf{A_2}{\Gamma_2}{E_2,K_2}{s_2'}{v_2}
                \\&\trans{\lpropret{i}}
                \conf{A_2}{\Gamma_2,\maps{i}{v_2}}{E_2,K_2}{s_2'}{\noe}
                \\&\trans{\lopret{\alpha}}
                \conf{A_2\uplus\alpha}{\Gamma_2,\maps{i}{v_2}}{K_2}{s_2'}{E_2\hole[\alpha]}
                &(\alpha\not\in\an{A_2,\Gamma_2,v_2,K_2,s_2',E_2})
                \\&\wtrans{\tau}
                \conf{A_2\uplus\alpha}{\Gamma_2,\maps{i}{v_2}}{K_2}{s_2''}{E_2'\hole[\app{\alpha}{v_2'}]}
                \\&\trans{\lpropapp{\alpha}{j}}
                \conf{A_2\uplus\alpha,\alpha'}{\Gamma_2,\maps{i}{v_2},\maps{j}{v_2'}}{E_2',K_2}{s_2''}{\noe}
                \\&\trans{\lopapp{i}{\alpha'}}
                \conf{A_2\uplus\alpha,\alpha'}{\Gamma_2,\maps{i}{v_2},\maps{j}{v_2'}}{E_2',K_2}{s_2''}{e_2'}
                &(\alpha'\not\in\an{A_2,\Gamma_2,v_2,v_2',E_2',K_2,s_2''})
               \\&=
                \begin{cases}
                  \conf{A_2\uplus\alpha,\alpha'}{\Gamma_2,\maps{i}{v_2},\maps{j}{v_2'}}{
                          E_2',K_2}{s_2''}{\app{\alpha''}{\alpha'}}
                                          &\rlap{\text{if } $v_2=\alpha''$}\\
                  \conf{A_2\uplus\alpha,\alpha'}{\Gamma_2,\maps{i}{v_2},\maps{j}{v_2'}}{
                          E_2',K_2}{s_2''}{\app{e_2'}\sub{x}{\alpha'}}
                                          &\rlap{\text{if } $v_2=\lam{x} e_2'$}
                \end{cases}
               \\&\wtrans{\tau}
               \conf{A_2\uplus\alpha,\alpha'}{\Gamma_2,\maps{i}{v_2},\maps{j}{v_2'}}{
                 E_2',K_2}{s_2'''}{e_2''} = C_4'
                & C_3' \simil C_4'
             \end{align*}
%             \begin{align*}
%               C_4 &= \conf{A_2}{\Gamma_2}{E_2,K_2}{s_2}{e_2}
%                \wtrans{\tau}
%                \conf{A_2}{\Gamma_2}{E_2,K_2}{s_2'}{v_2}
%                \\&\trans{\lpropret{i}}
%                \conf{A_2}{\Gamma_2,\maps{i}{v_2}}{E_2,K_2}{s_2'}{\noe}
%                \\&\trans{\lopret{\alpha}}
%                \conf{A_2\uplus\alpha}{\Gamma_2,\maps{i}{v_2}}{K_2}{s_2'}{E_2\hole[\alpha]}
%                &(\alpha\not\in\an{A_2,\Gamma_2,v_2,K_2,s_2',E_2})
%                \\&\wtrans{\tau}
%                \conf{A_2\uplus\alpha}{\Gamma_2,\maps{i}{v_2}}{K_2}{s_2''}{e_2'}
%                =C_4'
%                & C_3' \simil C_4'
%             \end{align*}
             \begin{align*}
               C_2 &= \conf{A_2}{\Gamma_2}{K_2}{s_2}{E_2[e_2]}
                \wtrans{\tau}
                \conf{A_2}{\Gamma_2}{E_2,K_2}{s_2'}{E_2[v_2]}
                \\&=
                \conf{A_2\uplus\alpha}{\Gamma_2}{K_2}{s_2'}{E_2\hole[\alpha]}
                \concr{\alpha}{v_2}
                \wtrans{\tau}
                \conf{A_2\uplus\alpha}{\Gamma_2}{K_2}{s_2''}{E_2'\hole[\app\alpha v_2']}
                \concr{\alpha}{v_2}
                \\&=
                \conf{A_2\uplus\alpha,\alpha'}{\Gamma_2}{K_2}{s_2''}{E_2'\hole[\app\alpha \alpha']}
                \concr{\alpha'}{v_2'}
                \concr{\alpha}{v_2}
                \\&
                \begin{cases}
                  =
                  \conf{A_2\uplus\alpha,\alpha'}{\Gamma_2}{K_2}{s_2''}{E_2'\hole[\app{\alpha''} \alpha']}
                  \concr{\alpha'}{v_2'}
                  \concr{\alpha}{v_2}
                                          &\rlap{\text{if } $v_2=\alpha''$}\\
                  \trans{\tau}
                  \conf{A_2\uplus\alpha,\alpha'}{\Gamma_2}{K_2}{s_2''}{E_2'\hole[e_2'\sub{x}{\alpha'}]}
                                          &\rlap{\text{if } $v_2=\lam{x} e_2'$}
                \end{cases}
               \\&\wtrans{\tau}
               \conf{A_2\uplus\alpha,\alpha'}{\Gamma_2}{K_2}{s_2'''}{E_2'\hole[e_2'']}
                  \concr{\alpha'}{v_2'}
                  \concr{\alpha}{v_2}
               = C_2'
             \end{align*}
%             \begin{align*}
%               C_2 &= \conf{A_2}{\Gamma_2}{K_2}{s_2}{E_2[e_2]}
%                \wtrans{\tau}
%                \conf{A_2}{\Gamma_2}{E_2,K_2}{s_2'}{E_2[v_2]}
%                \\&=
%                \conf{A_2\uplus\alpha}{\Gamma_2}{K_2}{s_2'}{E_2\hole[\alpha]}
%                \concr{\alpha}{v_2}
%                \wtrans{\tau}
%                \conf{A_2\uplus\alpha}{\Gamma_2}{K_2}{s_2''}{e_2'}
%                \concr{\alpha}{v_2}
%                =C_2'
%             \end{align*}
             Moreover: $C'_1 \utfolde*{\utfoldv{\utfoldv{\simil}}} C'_2$, as required.

            \item $F=\app v \hole$: Here it must be $v = \lam{x} e_{11}$ and $e'=e_{11}\sub{x}{v_1}$.
              By the LTS and $C_3\simil C_3'$ we have:
             \begin{align*}
               C_3 &= \conf{A_1}{\Gamma_1}{E\hole[F],K_1}{s_1}{v_1}
                \\&\trans{\lpropret{i}}
                \conf{A_2}{\Gamma_1,\maps{i}{v_1}}{E\hole[F],K_1}{s_1}{\noe}
                \\&\trans{\lopret{\alpha}}
                \conf{A_1\uplus\alpha}{\Gamma_1,\maps{i}{v_1}}{K_1}{s_1}{E\hole[\app {(\lam{x}{e_{11}})} \alpha]}
                \\&\trans{\tau}
                \conf{A_1\uplus\alpha}{\Gamma_1,\maps{i}{v_1}}{K_1}{s_1}{E\hole[e_{11}\sub{x}{\alpha}]}
                =C_3'
                &(\alpha\not\in\an{A_1,\Gamma_1,v_{1},K_1,s_1,E,v_1})
             \end{align*}
             \begin{align*}
               C_4 &= \conf{A_2}{\Gamma_2}{E_2,K_2}{s_2}{e_2}
                \wtrans{\tau}
                \conf{A_2}{\Gamma_2}{E_2,K_2}{s_2'}{v_2}
                \\&\trans{\lpropret{i}}
                \conf{A_2}{\Gamma_2,\maps{i}{v_2}}{E_2,K_2}{s_2'}{\noe}
                \\&\trans{\lopret{\alpha}}
                \conf{A_2\uplus\alpha}{\Gamma_2,\maps{i}{v_2}}{K_2}{s_2'}{E_2\hole[\alpha]}
                &(\alpha\not\in\an{A_2,\Gamma_2,v_2,K_2,s_2',E_2})
                \\&\wtrans{\tau}
                \conf{A_2\uplus\alpha}{\Gamma_2,\maps{i}{v_2}}{K_2}{s_2''}{e_2'}
                =C_4'
                & C_3' \simil C_4'
             \end{align*}
             \begin{align*}
               C_2 &= \conf{A_2}{\Gamma_2}{K_2}{s_2}{E_2[e_2]}
                \wtrans{\tau}
                \conf{A_2}{\Gamma_2}{E_2,K_2}{s_2'}{E_2[v_2]}
                \\&=
                \conf{A_2\uplus\alpha}{\Gamma_2}{K_2}{s_2'}{E_2\hole[\alpha]}
                \concr{\alpha}{v_2}
                \wtrans{\tau}
                \conf{A_2\uplus\alpha}{\Gamma_2}{K_2}{s_2''}{e_2'}
                \concr{\alpha}{v_2}
                =C_2'
             \end{align*}
             Moreover, $C_1' \utfoldv*{\simil} C_2'$.
  
           \item $F=l \asgn \hole$: Here $e'=\true$ and $s_1'=s_1\stupd{l}{v_1}$.
              By the LTS and $C_3\simil C_3'$ we have:
             \begin{align*}
               C_3 &= \conf{A_1}{\Gamma_1}{E\hole[F],K_1}{s_1}{v_1}
                \\&\trans{\lpropret{i}}
                \conf{A_2}{\Gamma_1,\maps{i}{v_1}}{E\hole[F],K_1}{s_1}{\noe}
                \\&\trans{\lopret{\alpha}}
                \conf{A_1\uplus\alpha}{\Gamma_1,\maps{i}{v_1}}{K_1}{s_1}{E\hole[l \asgn \alpha]}
                \\&\trans{\tau}
                \conf{A_1\uplus\alpha}{\Gamma_1,\maps{i}{v_1}}{K_1}{s_1\stupd{l}{\alpha}}{E\hole[\true]}
                =C_3'
                &(\alpha\not\in\an{A_1,\Gamma_1,v_{1},K_1,s_1,E,v_1})
             \end{align*}
             \begin{align*}
               C_4 &= \conf{A_2}{\Gamma_2}{E_2,K_2}{s_2}{e_2}
                \wtrans{\tau}
                \conf{A_2}{\Gamma_2}{E_2,K_2}{s_2'}{v_2}
                \\&\trans{\lpropret{i}}
                \conf{A_2}{\Gamma_2,\maps{i}{v_2}}{E_2,K_2}{s_2'}{\noe}
                \\&\trans{\lopret{\alpha}}
                \conf{A_2\uplus\alpha}{\Gamma_2,\maps{i}{v_2}}{K_2}{s_2'}{E_2\hole[\alpha]}
                &(\alpha\not\in\an{A_2,\Gamma_2,v_2,K_2,s_2',E_2})
                \\&\wtrans{\tau}
                \conf{A_2\uplus\alpha}{\Gamma_2,\maps{i}{v_2}}{K_2}{s_2''}{e_2'}
                =C_4'
                & C_3' \simil C_4'
             \end{align*}
             \begin{align*}
               C_2 &= \conf{A_2}{\Gamma_2}{K_2}{s_2}{E_2[e_2]}
                \wtrans{\tau}
                \conf{A_2}{\Gamma_2}{E_2,K_2}{s_2'}{E_2[v_2]}
                \\&=
                \conf{A_2\uplus\alpha}{\Gamma_2}{K_2}{s_2'}{E_2\hole[\alpha]}
                \concr{\alpha}{v_2}
                \wtrans{\tau}
                \conf{A_2\uplus\alpha}{\Gamma_2}{K_2}{s_2''}{e_2'}
                \concr{\alpha}{v_2}
                =C_2'
             \end{align*}
             Moreover, $C_1' \utfoldv*{\simil} C_2'$.

            \item $F=\cond{\hole}{e_{11}}{e_{12}}$:
              Here $v_1=\true$ or $v_1=\false$, and $e'=e_{11}$ or $e'=e_{12}$, respectively.
              In both sub-cases, the proof proceeds as in the case where $F=\arithop{\vec c_{11},\hole,\vec c_{12}}$.

          \end{itemize}

      \end{itemize}

  \end{itemize}

{\flushleft
  \iref{utfe2}: In this case we have:}
      $C_1 = \conf{A_1}{\Gamma_1}{K_{11},E'_1\hole[E_1],K_{12}}{s_1}{\hat e_1}$ and
      $C_2 = \conf{A_2}{\Gamma_2}{K_{21},E'_2\hole[E_2],K_{22}}{s_2}{\hat e_2}$ and
      $C_3 = \conf{A_1}{\Gamma_1}{K_{11},E_1,E'_1,K_{12}}{s_1}{\hat e_1}$ and
      $C_4 = \conf{A_2}{\Gamma_2}{K_{21},E_2,E'_2,K_{22}}{s_2}{\hat e_2}$ and
      $\sizeof{K_{11}}=\sizeof{K_{21}}$ and $C_3 \simil C_4$.
%
      When $\sizeof{K_{11}}>0$, because $C_1$ ($C_3$) and $C_2$ (resp.~ $C_4$) have the same expressions, 
      the proof requires a simple simulation diagram chasing, with the resulting configurations related in
      $\utfolde{\simil}$ via rule \iref{utfe2}.
      Similarly when $\eta \not\in\{\lopret{c},\lopret{\alpha}\where \text{any } c, \alpha$.
      When $\eta \in\{\lopret{c},\lopret{\alpha}\where \text{any } c, \alpha$, the simulation diagram is
      similar, but completed by relating the resulting configurations in
      $\utfolde{\simil}$ via rule \iref{utfe1}.
      Note that a $\lterm$-transition is not possible from $C_1$.


{\flushleft
  \iref{utfd1},
  \iref{utfd2}:}
  The proof in these cases proceeds as the corresponding cases above, with the simplification that the right-hand side configurations ($C_2$ and $C_4$) perform the required transitions via the LTS rule \iref{dummy}.
\end{proof}
%}}}

\begin{lemma}\label{lem:utfoldv-sound} %{{{
  Let $f= \utfolde{}\sqcup\utfoldv{}$
  and $g=\utperm{}$; then
  $\utfoldv{}\comp{\constf{\gfp\WP}}\progress(f\sqcup g)^\omega\comp{\constf{\gfp\WP}}$.
\end{lemma}
\begin{proof}
  We need to show
  $\utfoldv{}\comp{\constf{\gfp\WP}}\comp\WP(\bisim{R}) \sqsubseteq 
  {\WP}\comp (f\sqcup g)^\omega\comp{\constf{\gfp\WP}}(\bisim{R})$.
  Because $\constf{\gfp\WP}$ is the constant function mapping its argument to $(\simil)$, we need to show
  $\utfoldv{}(\simil) \sqsubseteq 
  {\WP}\comp (f\sqcup g)^\omega(\simil)$.

  Let $C_1\utfoldv*{\simil}C_2$, 
  and $C_1\trans{\eta}C_1'$.
  If $C_1\trans{\eta}C_1'$ is produced by rule \iref{dummy} then the proof is trivial as $C_2$ can perform the same transition and $C_1'=\botconf \utId*{\simil} \botconf=C_2'$. We thus consider only non-\iref{dummy} transitions from $C_1$.
  By case analysis, the derivation
  $C_1\utfoldv*{\simil}C_2$ can be produced by the \iref{utfv} or the \iref{utfd3} rules. We show the former; the proof of the latter is similar but simpler.

  {\flushleft
  \iref{utfv}:}
  Here we have
      $C_1 = C_3\kappa_1$ and
      $C_2 = C_4\kappa_2$ and
      $C_3=\conf{A_3\uplus\alpha}{\Gamma_3,\maps{i}{v_3}}{K_3}{s_3}{\hat e_3}$ and
      $C_4=\conf{A_4\uplus\alpha}{\Gamma_4,\maps{i}{v_4}}{K_4}{s_4}{\hat e_4}$ and
      $C_3 \simil C_4$ and
      $\alpha\not\in\an{v_3,v_4}$ and
      $\kappa_1=\concr{\alpha}{v_3}$ and
      $\kappa_2=\concr{\alpha}{v_4}$.
   We proceed by cases on the transition from $C_1$. Cases \iref{propretf}, \iref{opretf}, and \iref{term} are straightforward and are proved using \cref{lem:lts-concr}.

   \begin{itemize}
     \item \iref{propappf}: Both cases are similar; here we show the latter.
       We have $\eta=\lpropapp{\alpha'}{j}$ and $\alpha\in A_3$ ($\alpha\not=\alpha'$) and
       $\hat e_3\kappa_1=E_1\hole[\app{\alpha'} u_1]$ and
       \[
          C_1=\conf{A_3}{\Gamma_3\kappa_1}{K_3\kappa_1}{s_3\kappa_1}{E_1\hole[\app{\alpha'} u_1]}
          \trans{\lpropapp{\alpha'}{j}}
          \conf{A_3}{\Gamma_3\kappa_1,\maps{j}{u_1}}{E_1,K_3\kappa_1}{s_3\kappa_1}{\noe}
          =C_1'
        \]
        We choose $j'\not\in\dom{\Gamma_3}\uplus i$
        and create the permutation $\pi=(j\bij j')$. We derive
       \[
          C_1=\conf{A_3}{\Gamma_3\kappa_1}{K_3\kappa_1}{s_3\kappa_1}{E_1\hole[\app{\alpha'} u_1]}
          \trans{\lpropapp{\alpha'}{j'}}
          \conf{A_3}{\Gamma_3\kappa_1,\maps{j'}{u_1}}{E_1,K_3\kappa_1}{s_3\kappa_1}{\noe}
          =C_1'\pi
        \]
        We consider cases on 
       $\hat e_3\kappa_1=E_1\hole[\app{\alpha'} u_1]$:
       \begin{itemize}
         \item
           $\hat e_3=E_3\hole[\app{\alpha'} u_3]$ and
           $E_1=E_3\kappa_1$ and $u_1=u_3\kappa_1$.
           In this case we have
           \begin{align*}
             C_3=\conf{A_3\uplus\alpha}{\Gamma_3,\maps{i}{v_3}}{K_3}{s_3}{E_3\hole[\app{\alpha'} u_3]}
             &\trans{\lpropapp{\alpha'}{j'}}
             \conf{A_3\uplus\alpha}{\Gamma_3,\maps{i}{v_3},\maps{j'}{u_3}}{E_3,K_3}{s_3}{\noe}
             =C_3'
           \end{align*}
           By $C_3 \simil C_4$ we have 
           $C_4 \wtrans{\lpropapp{\alpha'}{j'}} C_4$ 
           and $C_3' \simil C_4'$.

           We have two cases. The first is when $C_4'=\botconf$. This case is straightforward using rule \iref{utfd3}
           and relating the resulting configurations in $\utperm{\utfoldv{\simil}}$.
           The other case is as follows.
           \begin{align*}
             C_4=\conf{A_4\uplus\alpha}{\Gamma_4,\maps{i}{v_4}}{K_4}{s_4}{\hat e_4}
             &\wtrans{\tau}
             \conf{A_4\uplus\alpha}{\Gamma_4,\maps{i}{v_4}}{K_4}{s_4'}{E_4\hole[\app{\alpha'} u_4]}
             \\
             &\trans{\lpropapp{\alpha'}{j'}}
             \conf{A_4\uplus\alpha}{\Gamma_4,\maps{i}{v_4},\maps{j'}{u_4}}{E_4,K_4}{s_4'}{\noe}
             =C_4'
             &\text{and } C_3' \simil C_4'
             \\
             C_2=\conf{A_4\uplus\alpha}{\Gamma_4,\maps{i}{v_4}}{K_4}{s_4}{\hat e_4}\kappa_2
             &\wtrans{\tau}
             \conf{A_4\uplus\alpha}{\Gamma_4,\maps{i}{v_4}}{K_4}{s_4'}{E_4\hole[\app{\alpha'} u_4]}\kappa_2
             &(\text{\ref{lem:lts-concr}})
             \\
             &\trans{\lpropapp{\alpha'}{j'}}
             \conf{A_4\uplus\alpha}{\Gamma_4,\maps{i}{v_4},\maps{j'}{u_4}}{E_4,K_4}{s_4'}{\noe}\kappa_2
             \\
              C_2
             &\wtrans{\lpropapp{\alpha'}{j}}
             C_4'\kappa_2\pi = C_2'
             &(\ref{lem:lts-perm})
            \end{align*}
            Moreover, $C_1' \utperm*{\utfoldv{\simil}} C_2'$, as required.
 
         \item $\hat e_3=E_3\hole[\app{\alpha} u_3]$ and
           $E_1=E_3\kappa_1$ and $u_1=u_3\kappa_1$ and $\kappa_1=\concr{\alpha}{\alpha'}$ and $v_3=\alpha$.
           In this case we have
           \begin{align*}
             C_3=\conf{A_3\uplus\alpha}{\Gamma_3,\maps{i}{v_3}}{K_3}{s_3}{E_3\hole[\app{\alpha} u_3]}
             &\trans{\lpropapp{\alpha}{j'}}
             \conf{A_3\uplus\alpha}{\Gamma_3,\maps{i}{v_3},\maps{j'}{u_3}}{E_3,K_3}{s_3}{\noe}
             =C_3'
           \end{align*}
           By $C_3 \simil C_4$ we have 
           $C_4 \wtrans{\lpropapp{\alpha}{j'}} C_4$ 
           and $C_3' \simil C_4'$.

           We have two cases. The first is when $C_4'=\botconf$. This case is straightforward using rule \iref{utfd3}
           and relating the resulting configurations in $\utperm{\utfoldv{\simil}}$.
           The other case is as follows.
           \begin{align*}
             C_4=\conf{A_4\uplus\alpha}{\Gamma_4,\maps{i}{v_4}}{K_4}{s_4}{\hat e_4}
             &\wtrans{\tau}
             \conf{A_4\uplus\alpha}{\Gamma_4,\maps{i}{v_4}}{K_4}{s_4'}{E_4\hole[\app\alpha u_4]}
             \\
             &\trans{\lpropapp{\alpha}{j'}}
             \conf{A_4\uplus\alpha}{\Gamma_4,\maps{i}{v_4},\maps{j'}{u_4}}{E_4,K_4}{s_4'}{\noe}
             =C_4'
             &\text{and } C_3' \simil C_4'
             \\
             C_2=\conf{A_4\uplus\alpha}{\Gamma_4,\maps{i}{v_4}}{K_4}{s_4}{\hat e_4}\kappa_2
             &\wtrans{\tau}
             \conf{A_4\uplus\alpha}{\Gamma_4,\maps{i}{v_4}}{K_4}{s_4'}{E_4\hole[\app\alpha u_4]}\kappa_2
             \\
             &\trans{\lpropapp{\alpha'}{j'}}
             \conf{A_4\uplus\alpha}{\Gamma_4,\maps{i}{v_4},\maps{j'}{u_4}}{E_4,K_4}{s_4'}{\noe}\kappa_2
             &(\text{\ref{lem:lts-concr}})
             \\
              C_2
             &\wtrans{\lpropapp{\alpha'}{j}}
             C_4'\kappa_2\pi = C_2'
             &(\ref{lem:lts-perm})
            \end{align*}
            Moreover, $C_1' \utperm*{\utfoldv{\simil}} C_2'$, as required.
        \end{itemize}
     \item \iref{opappf}: Both cases are similar; here we show the latter.
       We have $\eta=\lopapp{i'}{\alpha'}$ and $\alpha' \not\in A_3$ and $\hat e_3=\noe$ and
       $\Gamma_3(i')=u_3$ and $\app{u_3\kappa_1} \alpha' \funred e_1'$ and
       \[
         C_1= \conf{A_3\uplus\alpha}{\Gamma_3,\maps{i}{v_3}}{K_3}{s_3}{\noe}\kappa_1
          \trans{\lopapp{i'}{\alpha'}}
          \conf{A_3\uplus\alpha'}{\Gamma_3\kappa_1}{K_3\kappa_1}{s_3\kappa_1}{e_1'}
          =C_1'
        \]
        We choose $\alpha''\not\in A\uplus \alpha$
        and create the permutation $\pi=(\alpha'\bij \alpha'')$.
        We derive:
       \[
         C_1= \conf{A_3\uplus\alpha}{\Gamma_3,\maps{i}{v_3}}{K_3}{s_3}{\noe}\kappa_1
          \trans{\lopapp{i'}{\alpha''}}
          \conf{A_3\uplus\alpha''}{\Gamma_3\kappa_1}{K_3\kappa_1}{s_3\kappa_1}{e_1''}
          =C_1'\pi
        \]
         with $\app{u_3\kappa_1} \alpha'' \funred e_1''$.
         We consider cases on $u_3$ and $v_3$:
         \begin{itemize}
           \item $u_3 = \alpha$ and
             $v_3 = \lam x e_3''$: we have $e_1''=e_3''\sub{x}{\alpha''} = e_3''\sub{x}{\alpha''}\kappa_1$ 
                 ($\alpha\not\in\an{v_3}\cup\alpha''$).
%
             \begin{align*}
               C_1= \conf{A_3\uplus\alpha}{\Gamma_3,\maps{i}{v_3}}{K_3}{s_3}{\noe}\kappa_1
               &\trans{\lopapp{i'}{\alpha''}}
                \conf{A_3\uplus\alpha,\alpha''}{\Gamma_3,\maps{i}{v_3}}{K_3}{s_3}{e_3''\sub{x}{\alpha''}}\kappa_1
               =C_1'\pi
               \\
               C_3=\conf{A_3\uplus\alpha}{\Gamma_3,\maps{i}{v_3}}{K_3}{s_3}{\noe}
               &\trans{\lopapp{i'}{\alpha''}}
               \conf{A_3\uplus\alpha,\alpha''}{\Gamma_3,\maps{i}{v_3}}{K_3}{s_3}{\app{\alpha} \alpha''}
               \\
               &\trans{\lpropapp{\alpha}{j}}
               \conf{A_3\uplus\alpha,\alpha''}{\Gamma_3,\maps{i}{v_3},\maps{j}{\alpha''}}{\hole,K_3}{s_3}{\noe}
               \\
               &\trans{\lopapp{i}{\alpha'''}}
               \conf{A_3\uplus\alpha,\alpha'',\alpha'''}{\Gamma_3,\maps{i}{v_3},\maps{j}{\alpha''}}{\hole,K_3}{s_3}
               {e_3''\sub{x}{\alpha'''}}
               =C_3'
            \end{align*}
                 By $C_3 \simil C_4$ we have two cases. The first is when
                 $C_4$ weakly matches these transitions and becomes
                 $C_4'=\botconf$, due to an application of the \iref{dummy} rule.
                 This case is proved using rule \iref{utfd3} and relating the resulting
                 configurations in $\utperm{\utfolde{\utfoldv{\utfoldv{\simil}}}}$.
                 The other case is as follows.

                 By \cref{lem:simil-properties}, $\hat e_4=\noe$ and
                 $\Gamma_4(i')=u_4$ and 
             we proceed by cases on $u_4$ and $v_4$:
           \begin{itemize}
             \item $u_4 = \alpha_4\not=\alpha$:
               This is not possible because then $C_4$ would not be able to match the second transition from $C_3$.

             \item $u_4 = \alpha$ and
             $v_4 = \lam x e_4''$: we have:
            \begin{align*}
               C_4=\conf{A_4\uplus\alpha}{\Gamma_4,\maps{i}{v_4}}{K_4}{s_4}{\noe}
               &\trans{\lopapp{i'}{\alpha''}}
               \conf{A_4\uplus\alpha}{\Gamma_4,\maps{i}{v_4}}{K_4}{s_4}{\app{\alpha}{\alpha''}}
               \\
               &\trans{\lpropapp{\alpha}{j}}
               \conf{A_4\uplus\alpha,\alpha''}{\Gamma_4,\maps{i}{v_4},\maps{j}{\alpha''}}{\hole,K_4}{s_4}{\noe}
               \\
               &\trans{\lopapp{i}{\alpha'''}}
               \conf{A_4\uplus\alpha,\alpha'',\alpha'''}{\Gamma_4,\maps{i}{v_4},\maps{j}{\alpha''}}
               {\hole,K_4}{s_4}{e_4''\sub{x}{\alpha'''}}
               \\
               &\wtrans{\tau}
               \conf{A_4\uplus\alpha,\alpha'',\alpha'''}{\Gamma_4,\maps{i}{v_4},\maps{j}{\alpha''}}{\hole,K_4}{s_4'}{e_4''}
               =C_4'
            \end{align*}
           and $C_3' \simil C_4'$.
            \begin{align*}
               C_2=\conf{A_4\uplus\alpha}{\Gamma_4,\maps{i}{v_4}}{K_4}{s_4}{\noe}\kappa_2
               &\trans{\lopapp{i'}{\alpha''}}
               \conf{A_4\uplus\alpha,\alpha'',\alpha'''}{\Gamma_4,\maps{i}{v_4},\maps{j}{\alpha''}}
               {K_4}{s_4}{e_4''\sub{x}{\alpha'''}}\kappa_2\kappa_4
               \\&\qquad\qquad\qquad\qquad\qquad\qquad\qquad\qquad\qquad\qquad(\kappa_4=\concr{\alpha'''}{\alpha''})
               \\
               &\wtrans{\tau}
               \conf{A_4\uplus\alpha,\alpha'',\alpha'''}{\Gamma_4,\maps{i}{v_4},\maps{j}{\alpha''}}{K_4}{s_4'}{e_4''}
               \kappa_2\kappa_4
               =C_2'\pi
               \\
               C_2&\trans{\lopapp{i'}{\alpha'}} C_2'
            \end{align*}
               Moreover we derive $C_1' \utperm*{\utfolde{\utfoldv{\utfoldv{\simil}}}} C_2'$.
  
             \item $u_4 = \alpha$ and
             $v_4 = \alpha_4 \in A_4$: The proof is as before with transitions:
            \begin{align*}
               C_4=\conf{A_4\uplus\alpha}{\Gamma_4,\maps{i}{v_4}}{K_4}{s_4}{\noe}
               &\trans{\lopapp{i'}{\alpha''}}
               \trans{\lpropapp{\alpha}{j}}
               \\
               &\trans{\lopapp{i}{\alpha'''}}
               \conf{A_4\uplus\alpha,\alpha'',\alpha'''}{\Gamma_4,\maps{i}{v_4},\maps{j}{\alpha''}}
               {\hole,K_4}{s_4}{\app {\alpha_4} \alpha'''}
               =C_4'
               \\
               C_2=\conf{A_4\uplus\alpha}{\Gamma_4,\maps{i}{v_4}}{K_4}{s_4}{\noe}\kappa_2
               &\trans{\lopapp{i'}{\alpha''}}
               \conf{A_4\uplus\alpha,\alpha'',\alpha'''}{\Gamma_4,\maps{i}{v_4},\maps{j}{\alpha''}}
               {K_4}{s_4}{\app{\alpha_4}\alpha'''}\kappa_2\kappa_4
               =C_2'\pi
               \\&\qquad\qquad\qquad\qquad\qquad\qquad\qquad\qquad\qquad\qquad(\kappa_4=\concr{\alpha'''}{\alpha''})
               \\
               C_2&\trans{\lopapp{i'}{\alpha'}} C_2'
            \end{align*}
           and $C_3' \simil C_4'$.
               Moreover we derive $C_1' \utperm*{\utfolde{\utfoldv{\utfoldv{\simil}}}} C_2'$.
 
             \item $u_4 = \lam x e_4$:
             In this case we derive:
            \begin{align*}
               C_4=\conf{A_4\uplus\alpha}{\Gamma_4,\maps{i}{v_4}}{K_4}{s_4}{\noe}
               &\trans{\lopapp{i'}{\alpha''}}
               \conf{A_4\uplus\alpha}{\Gamma_4,\maps{i}{v_4}}{K_4}{s_4}{e_4\sub{x}{\alpha''}}
               \\
               &\wtrans{\tau}
               \conf{A_4\uplus\alpha}{\Gamma_4,\maps{i}{v_4}}{K_4}{s_4'}{E_4\hole[\app{\alpha}{w_4}]}
               \\
               &\trans{\lpropapp{\alpha}{j}}
               \conf{A_4\uplus\alpha,\alpha''}{\Gamma_4,\maps{i}{v_4},\maps{j}{w_4}}{E_4,K_4}{s_4}{\noe}
               \\
               &\trans{\lopapp{i}{\alpha'''}}
               \conf{A_4\uplus\alpha,\alpha'',\alpha'''}{\Gamma_4,\maps{i}{v_4},\maps{j}{w_4}}
               {E_4,K_4}{s_4}{e_4'}
               &(\app{v_4}{\alpha'''}\funred e_4')
               %\\&\qquad\qquad\qquad\qquad\qquad\qquad(\app{v_4}{\alpha'''}\funred e_4')
               \\
               &\wtrans{\tau}
               \conf{A_4\uplus\alpha,\alpha'',\alpha'''}{\Gamma_4,\maps{i}{v_4},\maps{j}{w_4}}{E_4,K_4}{s_4'}{e_4''}
               =C_4'
            \end{align*}
           and $C_3' \simil C_4'$.
            \begin{align*}
               C_2=\conf{A_4\uplus\alpha}{\Gamma_4,\maps{i}{v_4}}{K_4}{s_4}{\noe}\kappa_2
               &\trans{\lopapp{i'}{\alpha''}}
               \conf{A_4\uplus\alpha}{\Gamma_4,\maps{i}{v_4}}{K_4}{s_4}{e_4\sub{x}{\alpha''}}\kappa_2
               \\
               &\wtrans{\tau}
               \conf{A_4\uplus\alpha}{\Gamma_4,\maps{i}{v_4}}{K_4}{s_4'}{E_4\hole[\app{\alpha}{w_4}]}
               \kappa_2
               &(\ref{lem:lts-concr})
               \\
               &\mathrel{({\trans{\tau}}\cup {=})}
               \conf{A_4\uplus\alpha,\alpha'',\alpha'''}{\Gamma_4,\maps{i}{v_4},\maps{j}{w_4}}
               {K_4}{s_4}{E_4\hole[e_4']}
               \kappa_2\kappa_4
               \\&\qquad\qquad\qquad(\kappa_4=\concr{\alpha'''}{w_4},
               (\app{v_4}{\alpha'''})\kappa_2\kappa_4\funred e_4'\kappa_2\kappa_4)
               \\
               &\wtrans{\tau}
               \conf{A_4\uplus\alpha,\alpha'',\alpha'''}{\Gamma_4,\maps{i}{v_4},\maps{j}{w_4}}{K_4}{s_4'}
               {E_4\hole[e_4'']}
               \kappa_2\kappa_4
               =C_2'\pi
               \\
               C_2
               &\wtrans{\lopapp{i'}{\alpha''}}
               C_2'
            \end{align*}
               Moreover we derive $C_1' \utperm*{\utfolde{\utfoldv{\utfoldv{\simil}}}} C_2'$.
           \end{itemize}

           \item $u_3 = \alpha$ and
             $v_3 = \alpha_3\in A_3$: 
             In this case we have $e_1''=\app{\alpha_3}\alpha''=(\app{\alpha_3}\alpha'')\kappa_1$
             ($\alpha_3\not=\alpha\not=\alpha'')$, and derive the transitions:
             \begin{align*}
               C_1= \conf{A_3\uplus\alpha}{\Gamma_3,\maps{i}{v_3}}{K_3}{s_3}{\noe}\kappa_1
               &\trans{\lopapp{i'}{\alpha''}}
                \conf{A_3\uplus\alpha,\alpha''}{\Gamma_3,\maps{i}{v_3}}{K_3}{s_3}{\app\alpha\alpha''}\kappa_1
               =C_1'\pi
               \\
               C_3= \conf{A_3\uplus\alpha}{\Gamma_3,\maps{i}{v_3}}{K_3}{s_3}{\noe}
               &\trans{\lopapp{i'}{\alpha''}}
                \conf{A_3\uplus\alpha,\alpha''}{\Gamma_3,\maps{i}{v_3}}{K_3}{s_3}{\app\alpha\alpha''}
               =C_3'
              \end{align*}
                 By $C_3 \simil C_4$ we have two cases. The first is when
                 $C_4$ weakly matches these transitions and becomes
                 $C_4'=\botconf$. This case is proved using rule \iref{utfd3} and relating the resulting
                 configurations in $\utperm{\utfoldv{\simil}}$.
                 The other case is as follows:
                 By \cref{lem:simil-properties}, $\hat e_4=\noe$ and
                 $\Gamma_4(i')=u_4$ and 
             \begin{align*}
               C_4= \conf{A_4\uplus\alpha}{\Gamma_4,\maps{i}{v_4}}{K_4}{s_4}{\noe}
               &\trans{\lopapp{i'}{\alpha''}}
                \conf{A_4\uplus\alpha,\alpha''}{\Gamma_4,\maps{i}{v_4}}{K_4}{s_4}{e_4}
                \wtrans{\tau}C_4'
               &((\app{u_4}{\alpha''})\funred e_4)
               \\
               C_2=C_4\kappa_2
               &\wtrans{\lopapp{i'}{\alpha''}}
               C_4'\kappa_2=C_2\pi
               &(\text{as above})
                \\
               C_2=C_4\kappa_2
               &\wtrans{\lopapp{i'}{\alpha'}}
               C_4'\kappa_2\pi=C_2
              \end{align*}
              Moreover $C_3' \simil C_4'$ and thus
              $C_1' \utperm*{\utfoldv{\simil}} C_2'$.
 
           \item $v_1 = \alpha_3\in A_3$: Here $\alpha_3\not=\alpha$ and the proof proceeds as in the previous case.
             The resulting configurations are again related in $\utperm{\utfoldv{\simil}}$.
           \item $u_3 = \lam x e_3$: similarly.
\end{itemize}
   
 



     \item \iref{tau}:
       Here we have $\eta=\tau$ and
       \[
         C_1 = \conf{A_3\uplus\alpha}{\Gamma_3,\maps{i}{v_3}}{K_3}{s_3}{\hat e_3}\kappa_1
         \trans{\tau}
         \conf{A_3}{\Gamma_3\kappa_1}{K_3\kappa_1}{s_3'\kappa_1}{e_1'}
         = C_1'
       \]
       We distinguish the case when $\hat e_3\kappa_1 \not= E_1\hole[\app{\lam x e_1'} u_1]$, for any $E_1$, $\lam{x}e_1'$, $u_1'$. This case is straightforward and follows from \cref{lem:lts-concr}.
       In the remaining case 
       we proceed by case analysis of the equality
       $\hat e_3\kappa_1 = E_1\hole[\app{\lam x e_1'} u_1]$:
       \begin{itemize}
         \item $\hat e_3 = E_3\hole[\app{\lam x e_3'} u_3]$ and $E_1=E_3\kappa_1$ and
           $\lam x e_1' = \lam x e_3'\kappa_1$ and $u_1 = u_3\kappa_1$ and $s_3=s_3'$.
           This case follows again from \cref{lem:lts-concr}.
         \item $\hat e_3 = E_3\hole[\app\alpha u_3]$ and $E_1=E_3\kappa_1$ and
           $v_3 = \lam x e_1'$ and $u_1 = u_3\kappa_1$ and $s_3=s_3'$.
           Here we have
           \begin{align*}
             C_3=
             \conf{A_3\uplus\alpha}{\Gamma_3,\maps{i}{v_3}}{K_3}{s_3}{E_3\hole[\app\alpha u_3]}
             &\trans{\lpropapp{\alpha}{j}}
             \conf{A_3\uplus\alpha}{\Gamma_3,\maps{i}{v_3},\maps{j}{u_3}}{E_3,K_3}{s_3}{\noe}
             \\
             &\trans{\lopapp{i}{\alpha'}}
             \conf{A_3\uplus\alpha,\alpha'}{\Gamma_3,\maps{i}{v_3},\maps{j}{u_3}}{E_3,K_3}{s_3}{e_1'\sub{x}{\alpha'}}
             =C_3'
           \end{align*}
                 By $C_3 \simil C_4$ we have two cases. The first is when
                 $C_4$ weakly matches these transitions and becomes
                 $C_4'=\botconf$. This case is proved using rule \iref{utfd3} and relating the resulting
                 configurations in $\utfolde{\utfoldv{\utfoldv{\simil}}}$.
                 The other case is as follows:
           \begin{align*}
             C_4=
             \conf{A_4\uplus\alpha}{\Gamma_4,\maps{i}{v_4}}{K_4}{s_4'}{\hat e_4}
             &\wtrans{\tau}
             \conf{A_4\uplus\alpha}{\Gamma_4,\maps{i}{v_4}}{K_4}{s_4'}{E_4\hole[\app\alpha u_4]}
             \\
             &\trans{\lpropapp{\alpha}{j}}
             \conf{A_4\uplus\alpha}{\Gamma_4,\maps{i}{v_4},\maps{j}{u_4}}{E_4,K_4}{s_4'}{\noe}
             \\
             &\trans{\lopapp{j}{\alpha'}}
             \conf{A_4\uplus\alpha,\alpha'}{\Gamma_4,\maps{i}{v_4},\maps{j}{u_4}}{E_4,K_4}{s_4'}{e_4'}
             &(\app{v_4}{\alpha'} \funred e_4')
             \\
             &\wtrans{\tau}
             C_4'
           \end{align*}
           and $C_3' \simil C_4'$. As above we can derive:
           \begin{align*}
             C_2=
             \conf{A_4\uplus\alpha}{\Gamma_4,\maps{i}{v_4}}{K_4}{s_4'}{\hat e_4}\kappa_2
             &\wtrans{\tau}
             \conf{A_4\uplus\alpha}{\Gamma_4,\maps{i}{v_4}}{K_4}{s_4'}{E_4\hole[\app\alpha u_4]}\kappa_2
             \\
             &\mathrel{({\trans{\tau}}\cup{=})}
             \conf{A_4\uplus\alpha,\alpha'}{\Gamma_4,\maps{i}{v_4},\maps{j}{u_4}}{K_4}{s_4'}
             {E_4\hole[e_4']}\kappa_2\kappa_4
             \\
             &\qquad\qquad\qquad\qquad\qquad
             (\kappa_4=\concr{\alpha'}{u_4}, (\app{v_4}{\alpha'})\kappa_2\kappa_4 \funred e_4'\kappa_2\kappa_4)
             \\
             &\wtrans{\tau}
             C_4'\kappa_2\kappa_4
           \end{align*}
           Moreover we derive $C_1' \utfolde*{\utfoldv{\utfoldv{\simil}}} C_2'$.
           \qedhere
          \end{itemize}

   \end{itemize}
 \end{proof}
%}}}

\begin{proposition}\label{prop:utfold-sound} %{{{
  Functions \utfolde{} and \utfoldv{} are sound up-to techniques.
\end{proposition}
\begin{proof}
  Consider $f=\utfolde{}\sqcup\utfoldv{}$. It suffices to show that $f$ is \WP-sound.
  By \cref{lem:prfs}~(\ref{lem:prfs-3}), it is sufficient to show
  \begin{align*}
    \utfolde{} \comp{\constf{\gfp\WP}}&\progress(f\sqcup g_1)^{\omega}\comp{\constf{\gfp\WP}} &\text{and}\\
    \utfoldv{} \comp{\constf{\gfp\WP}}&\progress(f\sqcup g_2)^{\omega}\comp{\constf{\gfp\WP}}
  \end{align*}
  where $g_1=\emptyset$ and $g_2=g=\utperm{}$.
  We have $g_i\sqsubseteq\companion$ by \cref{lem:upto-perm}.
  We finally establish the needed progressions by \cref{lem:utfolde-sound,lem:utfoldv-sound}.
\end{proof}
%}}}

\subsection{Up to Context}
\todo{This section now requires no proof. Some content will move into the main paper, the rest to be removed.}

\begin{figure*}[t] %{{{

  \[\begin{array}{@{}c@{}}
    \irule[UpToCxt${}_s$][uptocxts]{
      \conf{A_1}{\Gamma_1}{K_1}{s_1}{\hat e_1}
      \bisim*{R}
      \conf{A_2}{\Gamma_2}{K_2}{s_2}{\hat e_2}
      \\
      \vec l \not\in\dom{s_1}\sqcup\dom{s_2}
      \\
      \fl{\vec v} \sqsubseteq \{\vec l\}
      \\
      \an{\vec v} \sqsubseteq A_1\cap A_2
    }{
      \conf{A_1}{\Gamma_1}{K_1}{s_1\stupd{\vec l}{\vec v}}{\hat e_1}
      \utcxt*[][\vec l]{\bisim{R}}
      \conf{A_2}{\Gamma_2}{K_2}{s_2\stupd{\vec l}{\vec v}}{\hat e_2}
    }
    \\\\
    \irule[UpToCxt${}_\Gamma$][uptocxtgamma]{
      \conf{A_1}{\Gamma_1}{K_1}{s_1}{\hat e_1}
      \utcxt*[][\vec l]{\bisim{R}}
      \conf{A_2}{\Gamma_2}{K_2}{s_2}{\hat e_2}
      \\
      i\not\in\dom{\Gamma_1}\sqcup\dom{\Gamma_2}
      \\
      \fl{v} \sqsubseteq \{\vec l\}
      \\
      \an{v} \sqsubseteq A_1\cap A_2
    }{
      \conf{A_1}{\Gamma_1,\maps{i}{v}}{K_{1}}{s_1}{\hat e_1}
      \utcxt*[][\vec l]{\bisim{R}}
      \conf{A_2}{\Gamma_2,\maps{i}{v}}{K_{2}}{s_2}{\hat e_2}
    }
    \\\\
    \irule[UpToCxt${}_K$][uptocxtk]{
      \conf{A_1}{\Gamma_1}{K_{11},K_{12}}{s_1}{\hat e_1}
      \utcxt*[][\vec l]{\bisim{R}}
      \conf{A_2}{\Gamma_2}{K_{21},K_{22}}{s_2}{\hat e_2}
      \\
      \sizeof{K_{11}}=\sizeof{K_{21}}
      \\
      \fl{E} \sqsubseteq \{\vec l\}
      \\
      \an{E} \sqsubseteq A_1\cap A_2
    }{
      \conf{A_1}{\Gamma_1}{K_{11},E,K_{12}}{s_1}{\hat e_1}
      \utcxt*[][\vec l]{\bisim{R}}
      \conf{A_2}{\Gamma_2}{K_{21},E,K_{21}}{s_2}{\hat e_2}
    }
    \\\\
    \irule[UpToCxt${}_e$][uptocxte]{
      \conf{A_1}{\Gamma_1}{K_1}{s_1}{\noe}
      \utcxt*[][\vec l]{\bisim{R}}
      \conf{A_2}{\Gamma_2}{K_2}{s_2}{\noe}
      \\
      \fl{e} \sqsubseteq \{\vec l\}
      \\
      \an{e} \sqsubseteq A_1\cap A_2
    }{
      \conf{A_1}{\Gamma_1}{K_1}{s_1}{e}
      \utcxt*[][\vec l]{\bisim{R}}
      \conf{A_2}{\Gamma_2}{K_2}{s_2}{e}
    }
    \\\\
    \utcxt{} = \displaystyle\bigcup_{\vec l} \utcxt[][\vec l]{}
  \end{array}\]
  \hrule
  \caption{Up-to context.}\label{fig:utcontext}
\end{figure*}
%}}}

\begin{lemma}
  Let 
  $g=
  \utId{}           % unused
  \sqcup\utperm{}     % unused
  \sqcup\utweak{}     % unused
  \sqcup\utgc{}       % unused
  \sqcup\utfolde{}    % unused
  \sqcup\utfoldv{}    % unused
  $; then
  $\utcxt[][\vec l]{}\comp{\constf{\gfp\WP}}\progress(\utcxt{}\sqcup g)^\omega\comp{\constf{\gfp\WP}}$.
\end{lemma}
\begin{proof}
  We need to show
  $\utcxt[][\vec l]{}\comp{\constf{\gfp\WP}}\comp\WP(\bisim{R}) \sqsubseteq 
  {\WP}\comp (\utcxt{}\sqcup g)^\omega\comp{\constf{\gfp\WP}}(\bisim{R})$.
  Because $\constf{\gfp\WP}$ is the constant function mapping its argument to $(\simil)$, we need to show
  $\utcxt[][\vec l]{}(\simil) \subseteq 
  {\WP}\comp (\utcxt{}\sqcup g)^\omega({\simil})$.
  
  %Let $C_1 \utcxt*[][\vec l]{\simil} C_2$ and $C_1 \trans{\eta} C_1'$. We need to show that there exists $C_2'$ such that 
  %$C_2 \wtrans{\eta} C_2'$ and $C_1' \bisim*{S} C_2'$, where $\bisim{S} = (\utcxt{}\sqcup g)^\omega(\simil)$.
  We proceed by induction on the derivation of $C_1 \utcxt*[][\vec l]{\simil} C_2$.

  {\flushleft
  \iref{uptocxts}:}
We have
$C_1 = \conf{A_1}{\Gamma_1}{K_1}{s_1\stupd{\vec l}{\vec v}}{\hat e_1}$ and
$C_2 = \conf{A_2}{\Gamma_2}{K_2}{s_2\stupd{\vec l}{\vec v}}{\hat e_2}$ and
$C_3 = \conf{A_1}{\Gamma_1}{K_1}{s_1}{\hat e_1}$ and
$C_4 = \conf{A_2}{\Gamma_2}{K_2}{s_2}{\hat e_2}$ and
$C_3 \simil C_4$ and
$\vec l \not\in\dom{s_1}\sqcup\dom{s_2}$ and
$\fl{\vec v} \sqsubseteq \{\vec l\}$ and
$\an{\vec v} \sqsubseteq A_1\cap A_2$.
  By \cref{def:asymp}, $C_1 \asymp C_3$ and $C_2 \asymp C_4$.
  Therefore $C_1 \utgc*{\simil} C_2$. By \cref{lem:utgc-sound},
  $C_1 \simil C_2$, thus
  $C_1 \mathrel{\WP\comp\utId{\simil}} C_2$, and finally
  $C_1 \mathrel{\WP\comp(\utcxt{}\cup g)^\omega(\simil)} C_2$.

  {\flushleft
  \iref{uptocxtgamma}:}
We have
$C_1 = \conf{A_1}{\Gamma_1,\maps{i}{v}}{K_{1}}{s_1}{\hat e_1}$ and
$C_2 = \conf{A_2}{\Gamma_2,\maps{i}{v}}{K_{2}}{s_2}{\hat e_2}$ and
$C_3 = \conf{A_1}{\Gamma_1}{K_1}{s_1}{\hat e_1}$ and
$C_4 = \conf{A_2}{\Gamma_2}{K_2}{s_2}{\hat e_2}$ and
$C_3 \utcxt*[][\vec l]{\bisim{R}} C_4$ and
$i\not\in\dom{\Gamma_1}\cup\dom{\Gamma_2}$ and
$\fl{v} \subseteq \{\vec l\}$ and
$\an{v} \subseteq A_1\cap A_2$.
  \todo[inline]{todo - Maybe up-to separation covers this lemma entirely!}

  
  Let $C_1 \utcxt*[][\vec l]{\simil} C_2$ and $C_1 \trans{\eta} C_1'$. We need to show that there exists $C_2'$ such that 
  $C_2 \wtrans{\eta} C_2'$ and $C_1' \bisim*{S} C_2'$, where $\bisim{S} = (\utcxt{}\cup g)^\omega(\simil)$.


  The proof is similar in the remaining two cases.
%    \irule[UpToCxt${}_K$][uptocxtk]{
%      \conf{A_1}{\Gamma_1}{K_{11},K_{12}}{s_1}{\hat e_1}
%      \utcxt*[][\vec l]{\bisim{R}}
%      \conf{A_2}{\Gamma_2}{K_{21},K_{22}}{s_2}{\hat e_2}
%      \\
%      \sizeof{K_{11}}=\sizeof{K_{21}}
%      \\
%      \fl{E} \sqsubseteq \{\vec l\}
%      \\
%      \an{E} \sqsubseteq A_1\cap A_2
%    }{
%      \conf{A_1}{\Gamma_1}{K_{11},E,K_{12}}{s_1}{\hat e_1}
%      \utcxt*[][\vec l]{\bisim{R}}
%      \conf{A_2}{\Gamma_2}{K_{21},E,K_{21}}{s_2}{\hat e_2}
%    }
%    \irule[UpToCxt${}_e$][uptocxte]{
%      \conf{A_1}{\Gamma_1}{K_1}{s_1}{\noe}
%      \utcxt*[][\vec l]{\bisim{R}}
%      \conf{A_2}{\Gamma_2}{K_2}{s_2}{\noe}
%      \\
%      \fl{e} \sqsubseteq \{\vec l\}
%      \\
%      \an{e} \sqsubseteq A_1\cap A_2
%    }{
%      \conf{A_1}{\Gamma_1}{K_1}{s_1}{e}
%      \utcxt*[][\vec l]{\bisim{R}}
%      \conf{A_2}{\Gamma_2}{K_2}{s_2}{e}
%    }
\qed
\end{proof}

\begin{lemma}
  $e_1 \cxteq e_2$ iff
  $\lam x e_1 \cxteq \lam x e_2$
\end{lemma}
\begin{proof}
  See Theorem 3.2 in \cite{KoutavasW06}.
\end{proof}
\begin{theorem}[Soundness of $\bisimil$]
  $e_1 \bisimil e_2$ implies $e_1 \cxteq e_2$.
\end{theorem}
\begin{proof}
  It suffices to show that $(bisimil)$ is a congruence.
  By the above lemma, it suffices to show that $(bisim)$ is a congruence for values.
  Let $v_1 \bisimil v_2$  and context $D$.
  We have
  \begin{align*}
    v_1 &\bisimil v_2
    \\
    \conf{\cdot}{\maps{i}{v_1}}{\cdot}{\cdot}{\cdot}
    &\bisimil
    \conf{\cdot}{\maps{i}{v_1}}{\cdot}{\cdot}{\cdot}
    &\text{ (by bisimulation def. and \iref{propretf} transition)}
    \\
    \conf{\alpha}{\maps{i}{v_1}}{\cdot}{\cdot}{\cdot}
    &\bisimil
    \conf{\alpha}{\maps{i}{v_2}}{\cdot}{\cdot}{\cdot}
    &\text{ (by soundness of $\utgc{\bisimil}$)}
    \\
    \conf{\alpha}{\maps{i}{v_1}}{\cdot}{\cdot}{D\hole[\alpha]}
    &\bisimil
    \conf{\alpha}{\maps{i}{v_2}}{\cdot}{\cdot}{D\hole[\alpha]}
    &\text{ (by soundness of $\utcxt{\bisimil}$)}
    \\
    \conf{\cdot}{\cdot}{\cdot}{\cdot}{D\hole[v_1]}
    &\bisimil
    \conf{\cdot}{\cdot}{\cdot}{\cdot}{D\hole[v_2]}
    &\text{ (by soundness of $\utfoldv{\bisimil}$)}
    \\
    D\hole[v_1] &\bisimil D\hole[v_2]
    &\text{ (by definition)}
  \end{align*}
  \qed

\end{proof}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main.tex"
%%% End:

